Searching Clinical Data Using Generative AI

Artificial Intelligence (AI) is making a major impact on healthcare, particularly through its application in natural language processing (NLP) and predictive analytics. The healthcare sector has increasingly adopted AI for tasks such as clinical data analysis and medical code assignment. However, searching for clinical information in large and often unorganized datasets remains a manual and error-prone process. Assisting this process with automations can help physicians improve their operational productivity significantly. In this paper, we present a generative AI approach, coined SearchAI, to enhance the accuracy and efficiency of searching clinical data. Unlike traditional code assignment, which is a one-to-one problem, clinical data search is a one-to-many problem, i.e., a given search query can map to a family of codes. Healthcare professionals typically search for groups of related diseases, drugs, or conditions that map to many codes, and therefore, they need search tools that can handle keyword synonyms, semantic variants, and broad open-ended queries. SearchAI employs a hierarchical model that respects the coding hierarchy and improves the traversal of relationships from parent to child nodes. SearchAI navigates these hierarchies predictively and ensures that all paths are reachable without losing any relevant nodes. To evaluate the effectiveness of SearchAI, we conducted a series of experiments using both public and production datasets. Our results show that SearchAI outperforms default hierarchical traversals across several metrics, including accuracy, robustness, performance, and scalability. SearchAI can help make clinical data more accessible, leading to streamlined workflows, reduced administrative burden, and enhanced coding and diagnostic accuracy.

==> related.tex <==
% !TeX root = journal.tex

\section{Related Work}
 
We now describe some of the related work in this area.
John Snow Labs evaluated the performance of modern Large Language Models (LLMs) in analyzing diagnostic descriptions and extracting ICD-10 codes. The study focused on John Snow Labs' Natural Language Processing (NLP), known as Spark NLP, and compared its performance with ChatGPT 3.5 and ChatGPT 4.0 through accuracy tests. Spark NLP achieved a 76\% success rate in assigning the correct ICD-10 codes, outperforming the ChatGPT models, where GPT 3.5 scored 40\% and GPT 4.0 scored 58\%~\cite{spark-nlp}.

Similarly, Miraico by ASUS is another software solution that leverages LLMs to analyze diagnoses and identify the correct ICD-10 codes. In their demo video, Miraico demonstrated its ability to process natural language, read text descriptions of patient diagnoses, and recommend matching ICD-10 codes. Medical professionals can input a diagnosis, and the AI assistant evaluates how closely it aligns with specific ICD-10 codes. According to their website, Miraico achieved 99.4\% accuracy in hospital deployments, and its AI recommendations demonstrated a recall rate of over 80\%~\cite{miraico}.

Both Spark NLP and Miraico have demonstrated high accuracy rates in ICD-10 coding, underscoring the potential of AI to improve coding reliability and reduce human error. Their success is largely attributed to the use of specialized datasets and domain-specific tasks tailored to the healthcare sector. For example, in the John Snow Labs experiment, LLMs like ChatGPT struggled to achieve high accuracy rates, whereas Spark NLP, which had undergone specific training and fine-tuning on healthcare-related data, performed significantly better. Miraico also benefited from its partnership with multiple hospitals and the processing of 340,000 medical records. The focus of these technologies on enhancing healthcare documentation highlights ongoing efforts to leverage AI for clinical efficiency and patient care.

Our focus in SearchAI is to provide a natural language search over clinical data. This could involve multiple codes as well as other structured data filters (e.g., demographics, test results, biomarkers, and so on). Users can combine multiple diseases (or drugs, tests, etc.) and SearchAI interprets the entire family of codes that are applicable. This makes the search problem different from the code assignment problem. Of course, SearchAI relies on the codes to be assigned in the first place, and hence it is orthogonal to other AI approaches. 

\balance

% \section{Quantum Technology}
 
 
% In addition to AI advancements in healthcare, we are also closely monitoring developments in quantum computing technology. Unlike traditional computers that use bits to represent values as 0 or 1, quantum computers leverage qubits, which can represent a 0, a 1, or any combination of both in superposition of both states. For instance, a classical computer would require millions of years to find the prime factors of a 2,048-bit number, whereas a quantum computer could accomplish the same task in just minutes. [6] 

 

% Currently, quantum computer technology is expensive, challenging to manufacture, and primarily accessible to accredited research institutions and large corporations. However, advancements are rapidly pushing this technology closer to public availability. One notable milestone came when Google unveiled its quantum computing chip, Willow, marking a breakthrough in quantum research. While the technology is still in its initial stages, its results are very surprising, as a task that would take Willow under 5 minutes to compute, would take the fastest supercomputer computer $10^{25}$ years or a timescale larger than the age of the universe. [7] 

 

% According to Ahmet Erdemir, PhD, Associate Staff at the Center for Computational Life Sciences, “AI methods are currently limited by the capabilities of classical computers in processing complex data. Quantum computing has the potential to enhance AI by overcoming limitations in data size, complexity, and speed of problem-solving.” [8] 

 

% Researchers at the Cleveland Clinic are already working on improving current AI methods in research by applying quantum computing techniques to protein structure prediction. Daniel Blankenberg, PhD, Assistant Staff, Center for Computational Life Sciences, talks about the potential for Quantum Computing in health sciences. This advanced technology can be utilized to find solutions for some of the most pressing challenges facing the medical field which previously could not be solved due to the limitations of classical computers in handling large datasets." “If we can overcome these limitations with quantum computing, it will revolutionize our ability to treat rare diseases and develop personalized medicine.” [8] 

 

% When it comes to solving the problem of ICD code lookup and drug prescription diagnoses, there are many complex computations involved that require the processing of vast amounts of medical data in real time. These computations span identifying the codes for diseases, and health conditions, searching for the correct treatment, cross-referencing them with patient histories, and ensuring compatibility with prescribed medications. Traditional computing systems, while powerful, can struggle with the sheer scale and complexity of this data, as they must handle a large volume of possible combinations. Quantum computing, with its ability to process large datasets simultaneously, could accelerate the search and retrieval of relevant medical codes and drug interactions. The ability to complete multiple tasks in parallel can help speed up the decision-making process, reduce errors, and overall improve the accuracy of the diagnosis. As the healthcare industry embraces data-driven solutions, the importance of quantum computing grows, and offers the potential to enhance how medical professionals interpret and apply critical information to patient care. 

